Web Agents with World Models: Learning and Leveraging Environment Dynamics in Web Navigation

Large language models (LLMs) have recently gained much attention in building autonomous agents. However, the performance of current LLM-based web agents in long-horizon tasks is far from optimal, often yielding errors such as repeatedly buying a non-refundable flight ticket. By contrast, humans can avoid such an irreversible mistake, as we have an awareness of the potential outcomes (e.g., losing money) of our actions, also known as the "world model". Motivated by this, our study first starts with preliminary analyses, confirming the absence of world models in current LLMs (e.g., GPT-4o, Claude-3.5-Sonnet, etc.). Then, we present a World-model-augmented (WMA) web agent, which simulates the outcomes of its actions for better decision-making. To overcome the challenges in training LLMs as world models predicting next observations, such as repeated elements across observations and long HTML inputs, we propose a transition-focused observation abstraction, where the prediction objectives are free-form natural language descriptions exclusively highlighting important state differences between time steps. Experiments on WebArena and Mind2Web show that our world models improve agents' policy selection without training and demonstrate our agents' cost- and time-efficiency compared to recent tree-search-based agents.

==> figure_latex/figure1_motivating_example.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.4\linewidth]{figure/figure1_motivating_example.pdf}
    \caption{ Figure 1 demonstrates the lack of state understanding in traditional language-guided web agents. In Figure 1(a), the agent fails to recognize the state change after the initial `click[33]' action and mistakenly repeats the same action instead of concluding the task. Figure 1(b) shows the average numbers of redundant actions repeated by agents within a single trajectory.}
    \label{fig:motivating_example}
\end{figure}

==> figure_latex/figure2_main_method.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\linewidth]{figure/figure2_main_method.pdf}
    \caption{Overview of an Environment-Dynamics-Aware (EDA) Web Agent correctly reasoning on state, using our comprehensive approach that integrates a pre-trained world model with (1) Next-state Prediction, (2) State-transition Verification, and (3) Transition-aware Action Prediction. Specifically, the agent uses the world model for (1) Next-state Prediction, anticipating the expected state update following an action such as `click [33]' (left). As the state transition occurs (right), the agent employs (2) State-transition Verification to check if the actual state change aligns with its prediction. This integrated approach, which includes reasoning on state transitions, enhance the agent's understanding of the current state, enabling it to accurately predict and perform the correct subsequent action, such as `click [6]'; hence, a (3) Transition-aware Action Prediction.}
    \label{fig:main_method}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/ablation_abstraction.tex <==
\begin{wraptable}[8]{r}{0.40\textwidth}
\vspace{-4mm}
\caption{Ablation results of transition-focused observation abstraction.}
\resizebox{0.40\textwidth}{!}{
\begin{tabular}{l|c}
\toprule
   \textbf{Method}  & \textbf{Success Rate}\\
\midrule
    Vanilla CoT & 7.1 \\
   w/o abstraction (\cref{ssec:observation-abstraction})  & - \\
   WMA (ours) & \textbf{8.3} \\
\bottomrule
\end{tabular}
}
% \vspace{-4mm}

\label{tab:ablation_abstraction}
\end{wraptable}

==> table/ablation_finetuning.tex <==
% \begin{table}[t]
% \centering
% \resizebox{0.65\linewidth}{!}{
% \begin{tabular}{ccc|c}
% \toprule
% Use World Model & World Model & Value Model & Success Rate  \\
% \midrule
% \textcolor{red}{\ding{55}} & -   & -  & 7.1    \\
% \textcolor{green}{\checkmark} & Prompted   & \textcolor{red}{\ding{55}}   & 7.4    \\
% \textcolor{green}{\checkmark} & Prompted   & \textcolor{green}{\checkmark}   & 6.3    \\
% \textcolor{green}{\checkmark} & Finetuned   & \textcolor{red}{\ding{55}}   & 5.9    \\
% \textcolor{green}{\checkmark} & Finetuned   & \textcolor{green}{\checkmark}   & \textbf{8.3}    \\
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation on the training world model and the choice of value function on WebArena}
% \label{tab:ablation_finetuning}
% \end{table}

\begin{table}[t]
\centering
\begin{minipage}{0.47\textwidth}
\caption{Ablation on the training world model using step-wise evaluation.}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lc|cc}
    \toprule
      \textbf{World Model}   & \textbf{Training} & \textbf{MRR} & \textbf{Hit@1} \\
      \midrule
      GPT-4o-mini   & \redcross &  55.90&  44.0\\
      GPT-4o   &  \redcross & 68.94  &  57.0\\
      WMA (ours)  & \greencheck & \textbf{75.82} & \textbf{67.0} \\
      \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_finetuning}
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}
\caption{Ablation on the training value model.}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lc|c}
    \toprule
      \textbf{Value Model}   & \textbf{Training} & \textbf{SR} \\
      \midrule
      GPT-4o-mini   & \redcross &  12.2 \\
      Llama-3.1-8B   &  \greencheck & 12.7\\
      \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_value_model}
\end{minipage}
\end{table}

==> table/num_sampled_action.tex <==
\begin{wraptable}[6]{r}{0.5\textwidth}
\vspace{-4mm}
\caption{Success rate (SR) and relative change over the baseline ($\Delta$) compared to the baseline ($k=1$) on Map domain.}
\label{tab:num_sampled_actions}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
    \textbf{$k$} & \textbf{1} & \textbf{3} & \textbf{5} & \textbf{7} & \textbf{9} \\
    \midrule
    SR & 7.1 & 17.0 & 16.1 & 21.4 & 20.5 \\
    $\Delta$ & - & +139\% & +127\% & +201\% & +189\% \\
\bottomrule
\end{tabular}
}
\end{wraptable}

% 7.1
% 17
% 16.1
% 21.4
% 20.5

==> table/prelim_analysis2.tex <==
\begin{wraptable}{r}{0.425\textwidth}

\caption{Results of the impact of the access to the outcome of action in action prediction.}
\centering

\resizebox{0.425\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{LLM} & \textbf{w/o next state} & \textbf{w/ next state} & $\Delta$ \\
\midrule
GPT-4o-mini & 41 & 53 & +29.2\% \\
GPT-4o & 51 & 70 & +37.2\% \\
GPT-4-turbo & 51 & 70 & +37.2\% \\
Claude-3.5 & 53 & 73 & +37.7\% \\
\bottomrule
\end{tabular}
}
\label{tab:prelim_analysis2}
\end{wraptable}

==> table/preliminary_analysis.tex <==
\begin{table*}[h]
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{lccc}
  \toprule
  \multirow{2}{*}{\textbf{LLM}} & \multirow{2}{*}{\textbf{Analysis I. Next State Prediction}} & \multicolumn{2}{c}{\textbf{Analysis II. Action Prediction}} \\
  \cmidrule(lr){3-4}
  & & \textbf{w/o next state} & \textbf{w/ next state} \\
  \midrule 
  GPT-4o-mini  & 54\% & 41 & - \\
  GPT-4o  & 55\% & 51 & - \\
  % & GPT-4~\citep{zhou2023webarena}  &  & 14.9\% & - & - \\
  GPT-4-Turbo  & 58\% & 51 & - \\
  Claude-Sonnet-3.5& 52\% & - & - \\
  \midrule
  Random  & 50\% & - & - \\
  Human  & 83\% & - & - \\
  \bottomrule
\end{tabular}
}
\caption{Performance of Language-guided Web Agents and Human Baseline on Next State Prediction and Action Prediction Tasks.}
\label{tab:prelim_results}
\end{table*}
% \begin{table*}[h]
% \centering
% \resizebox{0.85\linewidth}{!}{%
% \begin{tabular}{lcc}
%   \toprule
%   \textbf{Agent Model} & \textbf{Analysis I. Next State Prediction} & \textbf{Analysis II. Action Prediction} \\
%   \midrule 
%   \ 
%   \midrule
%   GPT-4o-mini~\citep{zhou2023webarena}  & 36\% & - \\
%   GPT-4o~\citep{zhou2023webarena}  &  -\% & - \\
%   % & GPT-4~\citep{zhou2023webarena}  &  & 14.9\% & - & - \\
%   Claude-Sonnet  &  -\% & - \\
%   Llama3  &  -\% & - \\
%   \midrule
%   Human  &  -\% & - \\
%   \bottomrule
% \end{tabular}
% }
% \caption{Performance of Language-guided Web Agents and Human Baseline on Next State Prediction and Action Prediction Tasks.}
% \label{tab:prelim_results}
% \end{table*}

==> table/ranking.tex <==
\begin{wraptable}[10]{r}{0.4\textwidth}
% \vspace{4mm}
\label{tab:ranking}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{l|ccc}
\toprule
   \textbf{Method}  & \textbf{MRR} & \textbf{Hit@1} & \textbf{Hit@3}\\
\midrule
   w/o $o_{t+1}$  & 0.47 & 0.24 & - \\
   WMA (ours) & \textbf{0.52} & \textbf{0.31} & - \\
\bottomrule
\end{tabular}
}
\caption{Step-wise evaluation results that show the importance of the access to the next state.}
% \vspace{-4mm}
\end{wraptable}

==> table/webarena_main_results.tex <==
\begin{table}[t!]
\vspace{-3mm}
\centering
\small
\caption{Task success rate on WebArena using \texttt{gpt-4}, and score breakdown on five website splits.}
\vspace{2mm}
\label{tab:webarena-results}
%
\begin{tabular}{l|c|ccccc|c}
\toprule
\multicolumn{1}{c|}{\bf Method} & {\bf Total SR} & {Shopping} & {CMS} & {Reddit} & {GitLab} & {Maps} & {\bf \# Steps} \\
\midrule
\multicolumn{8}{c}{\it With human engineered workflows} \\
{*SteP \citep{sodhi2023heap}} & {33.0} & {\bf 37.0} & {24.0} & {\bf 59.0} & {\bf 32.0} & {30.0} & {-} \\
\midrule
\multicolumn{8}{c}{\it Autonomous agent only} \\
{WebArena \citep{zhou2024webarena}} & {14.9} & {14.0} & {11.0} & {~6.0} & {15.0} & {16.0} & {-} \\
{AutoEval \citep{pan2024autonomous}} & {20.2} & {25.5} & {18.1} & {25.4} & {28.6} & {31.9} & {46.7} \\
{BrowserGym \citep{drouin2024workarena}} & {23.5} & {-} & {-} & {-} & {-} & {-} & {-} \\
{BrowserGym$_{\it ax-tree}$} & {15.0} & {17.2} & {14.8} & {20.2} & {19.0} & {25.5} & {~~7.9} \\
% \textsc{AWM$_{\it rule}$ (ours)} & {\bf 35.6} & {33.2} & {\bf 30.2} & {50.9} & {30.8} & {40.5} & {~~6.3} \\
\textsc{AWM (ours)} & {35.5} & {30.8} & {29.1} & {50.9} & {31.8} & {\bf 43.3} & {\bf ~~5.9} \\
\midrule
\textsc{AWM + WMA (ours)} & {35.5} & {30.8} & {29.1} & {50.9} & {31.8} & {\bf 43.3} & {\bf ~~5.9} \\
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

